Machine Learning model for gas-liquid interface reconstruction in CFD numerical simulations

The volume of fluid (VoF) method is widely used in multi-phase flow simulations to track and locate the interface between two immiscible fluids. A major bottleneck of the VoF method is the interface reconstruction step due to its high computational cost and low accuracy on unstructured grids. We propose a machine learning enhanced VoF method based on Graph Neural Networks (GNN) to accelerate the interface reconstruction on general unstructured meshes. We first develop a methodology to generate a synthetic dataset based on paraboloid surfaces discretized on unstructured meshes. We then train a GNN based model and perform generalization tests. Our results demonstrate the efficiency of a GNN based approach for interface reconstruction in multi-phase flow simulations in the industrial context.

==> sections/gnn.tex <==

\section{Graph Neural Network Model}
\label{sec:gnn}

% {\color{red}
% How  does GNN work?
% 
% Present the graph data structure (vertices, edges,...) GNN operators, GNN network, message passin concepts,...
% 
% Present Pytorch, Pytorch Geometric, SAGEConv,...
% 
% 
% Present Optuna,...
% }


In VoF methods, standard gaz-liquid interface reconstruction algorithms are computing expensive. The Machine Learning based approaches, proposed by Qi et al. in \cite{qi2019computing}, 
Patel et al. in \cite{patel2019computing} and Svyetlichnyy in \cite{svyetlichnyy2018neural}, handle only regular structured grids with classical feed-forward Artificial Neural Network (ANN) or Convolutional Neural Network (CNN) methods. In this paper, we extend these works to general 3D unstructured grid by introducing a new method based on Graph Neural Networks (GNNs). In this section, after a brief introduction to machine learning techniques based on ANNs and CNNs, we present GNNs methods that generalize CNNs to unstructured data. We then present the architecture of the network we have designed to build a prediction model of the interface geometrical properties.

\subsection{GNN models}


%Graph Neural Network (GNN) is the key element in our work. In this chapter, we will begin with the brief introduction about machine learning and then we will talk about GNNs as well as graphs on which GNNs are based on.

Machine Learning is a type of computer algorithms that can learn automatically from experience with the help of data. The algorithms build build a model with the data in the process called ``training". This enables to perform inference/prediction on new data. The quality of the inference is measured by a ``loss function", basically means the gap between the result of an inference and the true value. Therefore building a good machine learning model consists on looking for way to minimize the loss function. Neural Networks (NNs) are a subset of machine learning and its structure is inspired by human brain. NNs are typically comprised of a few linear layers of nodes (input, hidden and output) layers as illustrated in Fig.~\ref{fig:mlp}. Data is fed to NNs the input layer and predictions are made at the output layer. Nodes of each layer are connected to another in neighbor layers with an associated weight and thread-holds (activation function). This is the most basic form of NNs which is called Multi Layer Perceptrons (MLPs). Convolutional Neural Networks, or CNNs have typically have a few convolution layers before linear layers at the end of the networks. Those convolution layers consist of convolution filters which are capable of capture a spatial relationship which allows to treat images, videos and also applicable to the time series analysis such as audio signals. While CNNs are one of the most popular NNs, their capacity is limited to Euclidean data (images, videos, etc.). In this type of data, each data element (\textit{e.g.} pixel) are ordered and distributed with a fixed-interval, such as structured meshes. Although in real life some data are formed in a non-Eucliden fashion, such as Social media networks and molecules. Those data are called graphs. Its data structure is undordered. Nodes are distributed with an unfixed interval. The number of neighbor nodes varies, such as unstructured meshes. The data we treat in this work correspond to this type of data.

\begin{figure}[!h]
    \centering
    \includegraphics[width=0.4\textwidth]{images/MLP.png}
    \caption{An example of Multi Layer Perceptrons (MLPs)}
    \label{fig:mlp}
\end{figure}

Here are the mathematical definition of a graph. A graph is consisting of edges and nodes. Basically, nodes are points and edges are lines connecting the nodes as illustrated in Fig.\ref{fig:schema_graph}. A graph can be denoted as $G=(V, E)$ where $V$ is a set of nodes ($\mathcal{V}={1, ...,n}$) and $E$ is a set of edges. $n$ is the number of nodes found in the graph. If we define a node as $v_i \in V$, an edge pointing from $v_j$ to $v_i$ can be defined as $e_{ij}=(u_i, v_j)\in$. The neighboring nodes of a node $v$ can be defined as $N(v)={u\in V|(v,u)\in E}$. The adjacency matrix $\mathbf{A}$ is a $n\cross n$ matrix with $A_{ij}=1$ if $e_{ij} \in E$ and $A_{ij}=0$ if $e_{ij} \notin E$. This can be denoted as $\mathbf{A} \in [0,1]^{n \cross n}$ Each node of a graph can have some attributes $\mathbf{X}$. Here, $\mathbf{X}\in \mathbf{R}^{n \cross d}$ is a node feature matrix, where $d$ is the dimension of a node feature vector. Moreover, $\mathbf{x}_v \in \mathbf{R}^{d}$ can be defined as the feature vector of a node $v$ (the vectors associated to nodes in Fig.\ref{fig:schema_graph}). A graph can also have edge attributes, but this treatment will not be used in this paper. 

\begin{figure}[!h]
    \centering
    \includegraphics[width=0.4\textwidth]{images/graph_example.png}
    \caption{Schematic diagram of a graph}
    \label{fig:schema_graph}
\end{figure}

Graph Neural Networks (GNNs) are designed to treat data in graph structures. The idea of GNNs is to determine the “node embedding” of each node, by looking at the information on its neighboring nodes. The basic idea behind node embedding approaches is to use dimension reduction techniques to distill the high-dimensional information about a node’s graph neighborhood into a dense vector embedding. The arrows in Fig.\ref{fig:schema_graph} visualize this concept. Nodes features of the neighborhood are ``looked at" by the node at the middle of the figure to build node embeddings on it. These node embeddings can then be fed to downstream machine learning systems and aid in tasks such as node classification, clustering, and link prediction. Many types of GNNs have been proposed (see \cite{wu2020comprehensive} and \cite{zhou2020graph}, for example). A type of GNNs, Convoluional Graph Neural Networks (ConvGNNs) generalize the operation of convolution from grid data to graph data. The main idea is to generate a node $v$’s representation by aggregating its own features $\mathbf{x}_v$ and neighbors’ features $\mathbf{x}_u$, where $u \in N(v)$. In our work we employ SAGEConv which is a variant of ConvGNNs proposed by Hamilton et al. \cite{Hamilton2017inductive}.

Most frameworks proposed prior to SAGEConv are \textit{transducive}. \textit{Transducive} approaches directly optimize the embeddings for each node using matrix-factorization-based objectives, and do not naturally generalize to unseen data, since they make predictions on nodes in a single, fixed graph. Whereas SAGEConv, an \textit{inductive} framework, learns a function that generates embeddings by sampling and aggregating features from a node’s local neighborhood. This mechanism allows SAGEConv to generate node embeddings efficiently for unseen data. SAGEConv learn the topological structure of each node’s neighborhood as well as the distribution of node features in the neighborhood. It is based on a concept called message-passing which consists of an aggregation and an update of node features at each node (this will be explained below). 

Below is the forward propagation algorithm of SAGEConv. The intuition behind this is that at each iteration, or search depth, nodes aggregate information from their local neighbors. Iteration of this allows nodes to get more information from further nodes. The entire graph $G(V, E)$ and input features for all nodes $\mathbf{x}_v \in \mathbf{R}^d, \forall v \in V$ are provided as input, where $d$ is the dimension of a node vector.

The outer for loop does the iteration on $k$, the depth of the search and $\mathbf{h}_k$ denotes a node’s representation at this step. The inner for loop iterates on nodes $v \in V$, in which the aggregation of the representation from the nodes in its immediate neighborhood, $\mathbf{h}_{u}^{k-1}, \forall u \in N(v)$ into $\mathbf{h}_{N(v)}^{k}$. The aggregation step refers to the previous step $k-1$. Input node features are defined as the $k=0$ representations. After the aggregation, the node's current representation $\mathbf{h}_{v}^{k}$ and the aggregated neighbor $\mathbf{h}_{N(v)}^{k-1}$ are concatenated. This concatenated vector is fed through a fully connected layer with nonlinear activation function $\sigma$, which transforms the representations to $\mathbf{h}_{N(v)}^{k}$ for the next step $k+1$. the final representations output at depth $K$ is $\mathbf{z}_{v}, \forall v \in V$.

\begin{algorithm}[!h]
\caption{SAGEConv embedding generation (forward propagation) algorithm}\label{alg:sage}

\textbf{Input: } Graph $G(V, E)$; input features $\{ \mathbf{x}_v, \forall v \in V \}$; depth $K$; weight matrices $\mathbf{W}^k$, $\forall k \in \{1,..., K\}$; activation function $\sigma$; differentiable aggregator functions $\operatorname{AGGREGATE}_k$, $\forall k \in \{1,...,K \}$; neighborhood function $N:v\rightarrow2^V$

\textbf{Output: } Vector representations $\mathbf{z}_v$ for all $v \in V$
\begin{algorithmic}[1]
\State $\mathbf{h}_{v}^{0} \leftarrow \mathbf{x}_{v}, \forall v \in V;$
\For{$k=1 \ldots K $}
    \For{$v \in V$}
        \State $\mathbf{h}_{N(v)}^{k} \leftarrow \operatorname{AGGREGATE}_{k}\left(\left\{\mathbf{h}_{u}^{k-1}, \forall u \in N(v)\right\}\right)$;
        \State $\mathbf{h}_{v}^{k} \leftarrow \sigma\left(\mathbf{W}^{k} \cdot \operatorname{CONCAT}\left(\mathbf{h}_{v}^{k-1}, \mathbf{h}_{N(v)}^{k}\right)\right)$
    \EndFor
\State $\mathbf{h}_{v}^{k} \leftarrow \mathbf{h}_{v}^{k} /\left\|\mathbf{h}_{v}^{k}\right\|_{2}, \forall v \in V$
\EndFor
\State $\mathbf{z}_{v} \leftarrow \mathbf{h}_{v}^{K}, \forall v \in V$
\end{algorithmic}
\end{algorithm}

A variety of aggregate architectures have been proposed. Mean, LSTM, Pooling aggregator are often used. We employ the Mean aggregator in our work. Fig.\ref{fig:mespa} shows the concept of a message-passing with mean aggregator. This is done by the following steps.

\begin{enumerate}
    \item \(\mathrm{mean}_{u \in {N}(v)} \mathbf{h}_{u}^{k-1} \):
    Calculate a mean of features stocked at the neighbors $u$ of the node $v$. This step corresponds to the aggregation. \\
    \item \(\mathbf{W}_{2} \cdot \mathrm{mean}_{u \in N(v)} \mathbf{h}_{u}^{k-1} \):
    Add a weight (\(\mathbf{W}_{2}\)) to this mean
    \item \(\mathbf{x}_{v}^{\prime}=\mathbf{W}_{1} \mathbf{h}_{v}^{k-1} +\mathbf{W}_{2} \cdot \mathrm{mean}_{u \in \mathcal{N}(v)} \mathbf{h}_{u}^{k-1}\):
    Add the transformed (weighted) features of $v$ to the weighted mean of $\mathbf{x}$, define a new feature on $v$. This step corresponds to the update. \\
    \item \(\mathbf{h}_{v}^{k} = \sigma \Big(\mathbf{W}_{1} \mathbf{h}_{v}^{k-1}+\mathbf{W}_{2} \cdot \mathrm{mean}_{u \in N(v)} \mathbf{h}_{u}^{k-1}\Big) \):
    Add an activation function to pass the new features to the next layer \\
\end{enumerate}


\begin{figure}[!h]
    \centering
    \includegraphics[width=0.2\textwidth]{images/message_passing.png}
    \caption{Message-passing around a node $v$}
    \label{fig:mespa}         
\end{figure}

Those descriptions above about graphs and GNNs are a short summary of \cite{wu2020comprehensive}, \cite{zhou2020graph} and \cite{Hamilton2017inductive}. More details are explained in their papers.

We use Pytorch and Pytorch Geometric as platforms to develop our GNNs based interface reconstruction algorithm, through Pytorch Lightning interface. For the hyper-parameter optimization (described below), Optuna is used. PyTorch is an open source deep learning framework on Python programs originally developed by Facebook's AI Research lab (FAIR). It provides Numpy-like tensor computing and GPU acceleration and programs are built on a type-based automatic differentiation system \cite{pytorch}. Its flexibility and ease-to-use make it one of the most popular among the similar frameworks. PyTorch Geometric is a library built upon PyTorch in order to easily write and train Graph Neural Networks (GNNs). In addition, it consists of easy-to-use mini-batch loaders for operating on many small and single giant graphs, multi GPU-support \cite{pytorch-geometric}. Pytorch Lightning is a lightweight wrapper (high-level interface) for Pytorch (and Pytorch Geometric) to simplify the usage and abstract the detail of training \cite{pytorch-lightning}. Optuna is a library for automatic hyper-parameter optimization. It's based on Bayesian algorithm called Tree-structured Parzen Estimator. It allows to search on numerical variables such as number of layers/nodes, learning rate as well as methodological variables such as optimization method (SGD, Adam, etc.). Optuna is widely used for its ease-to-implement and user-friendly interface. 


{\color{red}

PRESENT Pytorch, Pytorch Geometric, SAGEConv,...

PRESENT Pytorch Lighning

}

\subsection{GNN4VoF architecture design}

\subsubsection{Data modelisation}
{\color{red}
Present the GNN4Fof architecture to predict interface geometric properties
\begin{itemize}
\item Graph features (vertices, edges) properties
\item surface properties
\end{itemize}
}

The surface reconstruction is performed in each single tetrahedron cell.
To reconstruct a surface in a tetrahedron cell, four surface properties need to be known; the normal, the curvature, the center and the area of the surface. Therefore we develop an algorithm to predict those properties. Fig.\ref{fig:properties} illustrates those four properties. The curvature is also a target though it is not drawn in the figure. Fig.\label{fig:graph} shows the surface to reconstruct and the graph on which the inference by GNNs is performed. Suppose that we want to reconstruct the interface between fluid A and B. The reconstruction is performed in terms of each small element in a cell (``surface of interest" in the figure). Tetrahedron meshes are formed around the interface. For simplicity, tetrahedron cells are expressed as triangles. A graph is formed around the interface. The gravity centers of each cell are defined as nodes. Let's call the cell containing the surface of interest ``center cell" and the node contained in it ``center node" in this paper. The nodes connected to the center node with a blue solid line share surfaces with the center cell, the nodes connected to the center node with a blue dotted line share a vertex with the center cell. We define those all nodes as neighbor nodes of the center cell. 

Basically our GNNs algorithm perform inference on the surface properties of a from the features of the graph nodes around the surface. Therefore to train the model, we need to have a dataset of which we know the surface properties and their corresponding feature. Concretely, we need to have the following variables.

\begin{description}
 \item Label: surface properties, \emph{i.e.}, normal, curvature, center and area
 \item Features: coordinates of vertices of a tetrahedron, edges, volume fraction
\end{description}

All the label variables should be stocked at the center node. And all the feature variables should be stocked at each of all the nodes in the graph. In the next subsection, data treatment such as matrix size of variables for each inference will be described in detail.

In the training algorithm, all the coordinates are normalized by the $L$ defined as $L = \textrm{max} (L_{x}, L_{y}, L_{z})$. $L_{x,y,z}$ is the longest length that the vertices of a tetrahedron cell can have in $x,y,z$. The idea behind this is to non-dimensionalize with the side length $L$ of a cube which can contain a tetrahedron. The curvature is non-dimensionalized as $H = LH'$ where $H'$ is the denationalized $H$, since the curvature has the dimension of an inverse radius. The area is non-dimensionalized as $S = S'/L^2$ where $S'$ is the dimensionalized $S$. The coordinates of the center $\mathbf{M}$ are expressed in the barycentric system as below.

\[\mathbf{M} = p_1 \mathbf{P}_1 + p_2 \mathbf{P}_2 + p_3 \mathbf{P}_3 + p_4 \mathbf{P}_4\]
where $\mathbf{P}_1, \mathbf{P}_2, \mathbf{P}_3, \mathbf{P}_4$ are the vectors each vertex of a tetrahedron (see Fig.\ref{fig:properties}). $p_1,p_2,p_3,p_4$ are coefficients which satisfy $p_1 + p_2 + p_3 + p_4 = 1$.

\begin{figure}[!h]
     \centering
     \begin{subfigure}[t]{0.40\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/properties.png}
         \caption{Surface properties}
         \label{fig:properties}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.59\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/graph.png}
         \caption{Graph structure}
         \label{fig:graph}     
     \end{subfigure}
     \caption{Gas-liquid interfaces representation with GNN graphs}
\end{figure}


\subsubsection{Neural network architecture}
Fig.\ref{fig:architecture} shows the architecture of our model. The model is composed of three different parts. The most challenging part of the predictions of all the surface properties is the normal. Defining the normal let us calculate the other properties. The quality of its prediction can affect the other properties too. Thus we designed an architecture that predicts the normal at first and progressively the other properties. To take advantage of the geometric information we have, NNs-1 (Neural Networks 1) predicts the normal and the curvature. NNs-1 takes the coordinates of vertices of tetrahedrons and the volume fraction $\alpha$ of each tetrahedron and the adjacency matrix $\mathbf{A}$. Concretely, at each node we have the $3$ dimensional coordinates for $4$ vertices of a tetrahedron $\{ \mathbf{P}_v \in \mathbf{R}^{3\cross4}, \forall v \in V \}$. Here coordinates of vertices are flattened in a manner that $\mathbf{P}_v = (x_1, y_1, z_1, x_2, y_2, ..., z_4)$ where $1,2,3,4$ are the number of vertex of a tetrahedron. Then it is concatenated with the volume fraction of the same node as $\mathbf{x}_v = \operatorname{CONCAT}\left( \alpha, \mathbf{P}_v \right) \in \mathbf{R}^{d=13}$. Therefore, an input feature of NNs-1 for a graph having $n$ nodes can be denoted as $\mathbf{X}_{1} \in \mathbf{R}^{13 \cross n}$. The adjacency matrix has the dimension of $\mathbf{A} \in [0,1]^{n \cross n}$. NNs-1 has two layers of SAGEConv at the beginning. \textcolor{red}{The longest distance for the message-passing is two edge-distances. This means that twice of message-passing is enough to collect all information (features) contained in a graph.} Then SAGEConv layers are followed by linear layers. They allow to reduce the number of nodes. A skip connection was applied on the first linear layer. This is expected to avoid over-fitting. Then a global-mean-pool comes after, which returns batch-wise averaged node features. After the series of layers, NNs-1 has a latent space, that is a representation of the compressed input data. The model diverges into two branches of linear layers for the prediction of the normal $\mathbf{N} \in \mathbf{R}^{3}$ and the curvature $H$.

NNs-2 is the model for the center prediction. For this, $\alpha$ and the coordinates of the vertices of the center node $\mathbf{P}_{center} \in \mathbf{R}^{3 \cross 4}$ and the normal $\mathbf{N}$ obtained by NNs-1 are used. $\mathbf{N}$ is fed in the form of the dot product with $\mathbf{P}_{center}$, that is, $\mathbf{N} \cdot \mathbf{P}_{center} \in \mathbf{R}^{4}$. This is to facilitate the neural network to find the surface indicating the resemblance between the normal and the vertex vector. Finally at the input, a concatenated form of them $\mathbf{X}_2 = \operatorname{CONCAT}\left( \alpha, \mathbf{N} \cdot \mathbf{P}_{center}, \mathbf{P}_{center} \right) \in \mathbf{R}^{17}$. At the output we will get the center $\mathbf{P} \in \mathbf{R}^3$. This model is composed by a series of linear layers.

NNs-3 is the model for the area prediction. The input is similar to the ones for NNs-2;  $\mathbf{X}_3 = \operatorname{CONCAT}\left( \mathbf{N} \cdot \mathbf{P}_{center}, \mathbf{P}_{center}, \mathbf{M} \right) \in \mathbf{R}^{19}$. Instead of the volume fraction, the center is fed. A sigmoid function is used after the final layer since the area is supposed to be $\sqrt{2}/2<1$ at most \textcolor{red}{(need to explain why)}.


\begin{figure}\centering
\subfloat[NN-1: Normal/Curvature]{\label{fig:nns1}\includegraphics[width=0.7\linewidth]{images/NNs1.png}}\par
\subfloat[NN-2: Center]{\label{fig:nns2}\includegraphics[width=0.7\linewidth]{images/NNs2.png}}\par
\subfloat[NN-3: Area]{\label{fig:nns3}\includegraphics[width=0.7\linewidth]{images/NNs3.png}}\par
\caption{Schematic diagram of the architecture, the numbers in the figure mean the number of node of the layer or the probability $p$ of dropout}
\label{fig:architecture}
\end{figure}
